Detector-Free Weakly Supervised Grounding by Separation

Nowadays, there is an abundance of data involving images and surrounding free-form text weakly corresponding to those images. Weakly Supervised phrase-Grounding (WSG) deals with the task of using this data to learn to localize (or to ground) arbitrary text phrases in images without any additional annotations. However, most recent SotA methods for WSG assume the existence of a pre-trained object detector, relying on it to produce the ROIs for localization. In this work, we focus on the task of Detector-Free WSG (DF-WSG) to solve WSG without relying on a pre-trained detector. We directly learn everything from the images and associated free-form text pairs, thus potentially gaining an advantage on the categories unsupported by the detector. The key idea behind our proposed Grounding by Separation (GbS) method is synthesizing `text to image-regions' associations by random alpha-blending of arbitrary image pairs and using the corresponding texts of the pair as conditions to recover the alpha map from the blended image via a segmentation network. At test time, this allows using the query phrase as a condition for a non-blended query image, thus interpreting the test image as a composition of a region corresponding to the phrase and the complement region. Using this approach we demonstrate a significant accuracy improvement, of up to $8.5\%$ over previous DF-WSG SotA, for a range of benchmarks including Flickr30K, Visual Genome, and ReferIt, as well as a significant complementary improvement (above $7\%$) over the detector-based approaches for WSG.

==> files/related_backup.tex <==
\section{Related Work}
Joint analysis of natural images and text is a basic component of many downstream tasks, such as image captioning \cite{cornia2020meshed, karpathy2015deep, pan2020x, vinyals2016show, wang2016image, yao2017boosting, you2016image, zhou2020unified} , text based image retrieval, visual question answering \cite{alberti2019fusion, antol2015vqa, chen2020counterfactual, gokhale2020vqa, goyal2017making,xu2016ask}, and visual language grounding.
Recently Radford \etal~\cite{radford2021learning} proposed a joint image-text learning approach for zero-shot image classification using contrastive learning for image-text pairs. 
% Image captioning is the task of automatically generating a plausible textual description of an image, such that the input is an image and the output is a textual description \cite{}. Text based image retrieval on the other hand tires to find an image, from a given corpus, which most closely matches a given textual description. In this case, the input is a piece of text and the output is an image \cite{}. VQA, is a more complex task of inferring the answer to a given question about a specific image. In this case, the input is an image and a textual question. The output is also a piece of text which should infer the correct answer to the question with respect to the given image, \cite{}.
We focus on the task of visual language grounding which aims to localize a textual phrase within a given image. In this task, the input is an image and several phrases describing parts of the image. The output is the location within the image corresponding to each phrase. 
% Image/video captioing: Image --> Text, VQA, Text-->Image-->Text, text based image retrieval: Text-->Image, Grounding --> Text --> Image localization §§

We make the distinction \shimon {between} if three types of supervision when training grounding model, i.e. fully supervised, weakly supervised, and \ourstaskfull{}. 
Fully supervised methods require the data to be annotated such that each phrase has a corresponding location within the image, usually in the form of a bounding box. 
Weakly supervised methods, on the other hand, do not require bounding box annotations for the given phrases but rather pairs of images and corresponding captions (textual descriptions of the image). However they do require a pre-trained object detector \shimon{detectors} in order to extract regions of interest (ROIs) from the image. 
These detectors are trained on a massive corpus of fully annotated data and can generate reliable proposals for objects within the image and thus perform most of the localization. 
We refer to a method as \ourstaskfull{} when the training data is comprised of pairs of images with corresponding captions \textbf{without} localization annotation and \textbf{without} utilizing pre-trained object detectors. In this scenario, the phrase localization is inferred solely from the weakly annotated data.

\subsection{Fully supervised methods}

Fully supervised methods aim to solve the grounding problem using an end to end training procedure where the annotations include pairs of phrases with their corresponding bonding box location. In their work, Plummer \etal~\cite{plummer2015flickr30k} present the Flickr30K dataset which is designed for fully supervised training, and propose a Canonical Corolation Analsys (CCA) model to learn the joint visual-textual representation space.  The probabilistic approach of Mao \etal~\cite{Mao_2016_CVPR} evaluated the maximum likelihood of a given phrase with respect to a model trained to generate the expressions for each ROI within the image. Other methods such as Chen \etal~\cite{chen2017msrc} advocate the use of context query phrases in order to localize a given phrase. In such a framework, a query is not only defined by the query phrase alone, but also requires additional query phrases (context) which act as negative examples during test time. In some cases, where the context is available this may be an advantage, however, if the context is unavailable this assumption may hinder the capabilities of the method. In the work of Chen \etal~\cite{chen2017query} the context of the query phrase is also used in a reinforcement-learning approach. This method leverages the semantic context information by jointly learning a bounding box proposal generation network, \shimon{add space}a query-guided regression network, and a context policy network in order to leverage the semantic context information.

\subsection{Weakly Supervised Methods}

Some recent methods, relax the full supervision and require only image level annotations in the form of captions. However, these methods assume the availability of a pre-trained object detector, which performs most of the localization. These methods generally aim to create a joint space from the representation of both the images and the textual phrases thus transforming the grounding objective into a retrieval objective. Datta \etal~\cite{datta2019align2ground} directly aim to maximize the cosine similarity of the ROI embeddings with the caption embeddings, while Gupta \etal~\cite{gupta2020contrastive} introduce a contrastive loss \shimon{remove 
'and',  fix the sentence}and by generating negative examples and aiming to maximize the mutual information between the positive pairs of ROI-caption embeddings.  
Wang \etal~\cite{wang2019phrase} propose an un-paired training regime where the \shimon{remove 'objects'}objects multiple pre-trained object detectors are used to extract object proposals, and the object label, as predicted by the detector, is compared to the query phrase. 
Recent methods aim to create a task-agnostic, joint representation space for images and text \cite{chen2020uniter, huang2020pixel, li2020unicoder, li2019visualbert, li2020weakly, lu2019vilbert, lu202012, su2019vl, sun2019videobert, tan2019lxmert, zhou2020unified}. These methods are evaluated on many multi-modal tasks while the application of these methods to phrase grounding is done using a pre-trained detector.

\subsection{Detector Free Weakly Supervised Methods} \shimon{use detector-free}

As opposed to WSG methods, \ourstask{} methods perform dense localization scores for a given query phrase. These method normally generate dense attention heatmaps as opposed to ranking ROIs. In these cases, the ``Pointing Game" accuracy measure is a natural fit for the method evaluation. Lacking any localization information, these methods often define and optimize some auxiliary task on the weakly supervised data. While the auxiliary task is not identical to the grounding objective, optimization of the task leads to the desired phrase grounding results. 

Xiao \etal~\cite{xiao2017weakly} propose a hierarchical sentence parsing approach and enforce structural and compositional similarities between the attended image regions and the corresponding phrase in the parsed sentence tree. 
Javed \etal~\cite{javed2018learning} jointly learn the visual representations of multiple images which share a specific concept (noun) in the caption. An attention mechanism is applied to the visual features and the auxiliary task tries to predict the concept of the attended region. 
Zhang \etal~ \cite{zhang2018top} build upon an image/video captioning model and extract saliency maps with respect to the desired query phrase. 
%This method does not directly train the model to perform language grounding but rather evaluate
The work of Akbari \etal~\cite{akbari2019multi}, currently the SotA \ourstask{} method, does not use an auxiliary task but rather train \shimon{trains} a joint feature space for the image and text embedding. A similarity measure is computed for multiple image scales and the most similar scale, per image-phrase pair, is selected for the heatmap generation.
Our work is an \ourstask{} methods which presents a novel auxiliary task of image separation. We further show the importance of regularization terms which support the auxiliary task and align the outcome to the desired phrase grounding objective. 



Blind source separation, which aims to separate source signals from a set of mixed ones, has been used in machine learning well before the revival of deep networks (). The success of deep neural networks in restoration and generation tasks has revived the interest of the community in the subject (). Most research effort in this field is devoted to audio (speech / music) source separation (), which usually use a “synthetic cocktail party” dataset, where the original signals, simultaneously predicted at test time, being used as ground truth. Some of works in this field also use visual cues to improve performance in a multi-modal setting (). Our primary application area is computer vision. Current methods in vision source separation includes supervised regression () or generative adversarial separation (), predicting original components or synthetic masks. (Also similar to mix-up regularization ()) (Another direction is Double-DIP () that separate superimposed images with a single observation at test time). 
Our work, on the other hand, performs visual source separation conditioned on caption ques during training on a “synthetic image-caption cocktail dataset”. The conditioning operation on train time allows us to implicitly learn (objects, labels) information used to visually grounding language concepts at test time (in complementary to other existing methods).

==> tables/alpha_ablation.tex <==
% \begin{table}
% \begin{center}
% \begin{tabular}{ c c|c }
% %  \hline
%  Perlin & Gaussian & Hit Accuracy\\ 
%  \hline
%  100\% & 0\% & 68.37 \\
% %  \hline
%  0\% & 100\% & 70.65\\
% %  \hline
%  50\% & 50\% & \textbf{72.6} \\
% %  \hline
% \end{tabular}
% \end{center}
% \caption{Comparison of different variants of alpha map generation and the percentage used to build the batched data. The evaluation was done using the ``pointing game" accuracy on Flickr30K. All the the networks where trained with BERT+VGG models.}
% \label{tab:alpha_ablation}
% \end{table}

\begin{table}
\begin{center}
\begin{tabular}{ ccc }
%  \hline
\toprule
 Perlin & Gaussian & Pointing Accuracy\\ 
 \midrule
 100\% & 0\% & 68.37 \\
%  \hline
 0\% & 100\% & 70.65\\
%  \hline
 50\% & 50\% & \textbf{72.6} \\
%  \hline
\bottomrule
\end{tabular}
\end{center}
\caption{Comparison of different variants of alpha map generation including their mix (in $\%$ of the batch size). 
% The evaluation was done using the ``pointing game" accuracy on Flickr30K. All the the networks where trained with BERT+VGG models.
}
\figvspace
\label{tab:alpha_ablation}
\end{table}


==> tables/detector_based_ablation.tex <==
\begin{table}
\begin{center}
\begin{tabular}{ l| c }
% \hline
 Method & Pointing Accuracy\\
 \midrule
  Align2Ground \cite{datta2019align2ground} & 71.00\\
  InfoGround \cite{gupta2020contrastive} & 76.74\\
  Ours + InfoGround &  \textbf{83.90}\\ 
\end{tabular}
\end{center}
\caption{Comparison to detector based methods. The last line is an ensemble of our best PNASNet network with the SotA InfoGround method \cite{gupta2020contrastive}}
\figvspace
\label{tab:detector_results}
\end{table}


==> tables/detector_detailed_backup.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{ l|| c |c c c c c c c c c }
% \hline
 Method & Overall &People & Animals & Vehicles & Instruments & Bodyparts & Clothing & Scene & Other \\
 \midrule
  Ours (VGG) & 72.6 & 82.5 & \textcolor{blue}{\textbf{91.5}} & 81.1 & 56.6 & 34.8 & 58.6 & 70.9 & 59.9 \\ 
  Ours (PNASNet) & 74.5 & \textcolor{blue}{\textbf{83.6}} & 89.3 & \textcolor{blue}{\textbf{92.1}} & \textcolor{blue}{\textbf{83.3}} & \textcolor{blue}{\textbf{53.2}} & 50.1 & 71.3 & 66.7 \\ 
  Align2Ground~\cite{datta2019align2ground}&71.0&-&-&-&-&-&-&-&-\\
  InfoGround (IG)~\cite{gupta2020contrastive} & \textcolor{blue}{\textbf{76.74}} & 83.2 & 89.7 & 87 & 69.7 & 45.1 & \textcolor{blue}{\textbf{74.5}} & \textcolor{blue}{\textbf{80.6}} & \textcolor{blue}{\textbf{67.3}} \\
  \midrule
  Ours (VGG) + IG &  \textbf{83.9} & \textbf{88.8} & \textbf{96.1} & 93.4 &74.4 & \textbf{65.2} & 77.2 & \textbf{82.4} & 76.8 \\
  Ours (PNASNet) + IG &  83.4 & 87.3 & 95.2 & \textbf{95.4} &\textbf{ 75.2}& 62.3 & \textbf{78.3} & 81.5 & \textbf{77.2} \\
\end{tabular}
\end{center}
\caption{Detailed comparison with detector-based WSG methods \cite{datta2019align2ground, gupta2020contrastive} on Flickr30K. The last two lines are an ensemble of our \oursspace models with the SotA InfoGround (IG) method \cite{gupta2020contrastive}. In \textcolor{blue}{\textbf{blue}} - best single model result, in \textbf{bold black} - best overall result.}
\label{tab:detector_detailed_results}
\end{table*}

==> tables/image2text_weight_ablation.tex <==
\begin{table}
\begin{center}
\begin{tabular}{ c| c c c }
% \hline
 Scale factor & 0.01 & 0.1 & 1\\ 
 \midrule
 Pointing Accuracy & 65.7 & \textbf{72.6} & 70.8  \\
\end{tabular}
\end{center}
\caption{\mgloss{} scale factor }
\figvspace
\label{tab:image2text_weight}
\end{table}

